Path Planning using Reinforcement Learning: A Policy Iteration Approach

With the impact of real-time processing being realized in the recent past, the need for efficient implementations of reinforcement learning algorithms has been on the rise. Albeit the numerous advantages of Bellman equations utilized in RL algorithms, they are not without the large search space of design parameters. This research aims to shed light on the design space exploration associated with reinforcement learning parameters, specifically that of Policy Iteration. Given the large computational expenses of fine-tuning the parameters of reinforcement learning algorithms, we propose an auto-tuner-based ordinal regression approach to accelerate the process of exploring these parameters and, in return, accelerate convergence towards an optimal policy. Our approach provides 1.82x peak speedup with an average of 1.48x speedup over the previous state-of-the-art.

==> util/word_count.tex <==
% __        __            _    ____                  _   
% \ \      / /__  _ __ __| |  / ___|___  _   _ _ __ | |_ 
%  \ \ /\ / / _ \| '__/ _` | | |   / _ \| | | | '_ \| __|
%   \ V  V / (_) | | | (_| | | |__| (_) | |_| | | | | |_ 
%    \_/\_/ \___/|_|  \__,_|  \____\___/ \__,_|_| |_|\__|


\begin{table}[ht]
	\centering % used for centering table
	\begin{tabular}{l c c} % centered columns (4 columns)
		\hline\hline %inserts double horizontal lines
		\textbf{Section} & \textbf{Word Count} & \textbf{Char Count} \\ [0.5ex] % inserts table
		%heading
		\hline % inserts single horizontal line
		Abstract & \quickwordcount{sections/01_abstract} & \quickcharcount{sections/01_abstract} \\
% 		Version 3 & 94.1\% \\ [1ex]
		\hline %inserts single line
	\end{tabular}
	\caption{Word counts for all sections} % title of Table
	\label{table:word_counts} % is used to refer this table in the text
\end{table}
